DWE+: Dual-Way Matching Enhanced Framework for Multimodal Entity Linking

Multimodal entity linking (MEL) aims to utilize multimodal information (usually textual and visual information) to link ambiguous mentions to unambiguous entities in knowledge base. Current methods facing main issues: (1)treating the entire image as input may contain redundant information. (2)the insufficient utilization of entity-related information, such as attributes in images. (3)semantic inconsistency between the entity in knowledge base and its representation. To this end, we propose DWE+ for multimodal entity linking. DWE+ could capture finer semantics and dynamically maintain semantic consistency with entities. This is achieved by three aspects: (a)we introduce a method for extracting fine-grained image features by partitioning the image into multiple local objects. Then, hierarchical contrastive learning is used to further align semantics between coarse-grained information(text and image) and fine-grained (mention and visual objects). (b)we explore ways to extract visual attributes from images to enhance fusion feature such as facial features and identity. (c)we leverage Wikipedia and ChatGPT to capture the entity representation, achieving semantic enrichment from both static and dynamic perspectives, which better reflects the real-world entity semantics. Experiments on Wikimel, Richpedia, and Wikidiverse datasets demonstrate the effectiveness of DWE+ in improving MEL performance. Specifically, we optimize these datasets and achieve state-of-the-art performance on the enhanced datasets. The code and enhanced datasets are released on https://github.com/season1blue/DWET

==> Tables/details.tex <==

% \begin{figure}[htbp]
% \centering
% \subfigure[pic1.]{
% \includegraphics[width=0.5\linewidth]{Figures/detail1.eps}
% %\caption{fig1}
% }
% \quad
% \subfigure[pic2.]{
% \includegraphics[width=0.5\linewidth]{Figures/detail2.eps}
% }
% \quad
% \subfigure[pic3.]{
% \includegraphics[width=0.5\linewidth]{Figures/detail3.eps}
% }
% \quad
% \subfigure[pic4.]{
% \includegraphics[width=0.5\linewidth]{Figures/detail4.eps}
% }
% \caption{Top-1 accuracy under different hyperparameters: (1)in batch negative number (2)batch size (3)weight of contrastive loss $\lambda_c$ (4)weight of triplet loss $\lambda_t$.}
% \label{fig:details}
% \end{figure}

\begin{figure} [htbp]
    \centering
    \subfloat[\label{subfig:a}]{
        \includegraphics[width=0.5\linewidth]{Figures/detail1.eps}}
    \hspace{-5mm}
    \subfloat[\label{subfig:b}]{
        \includegraphics[width=0.5\linewidth]{Figures/detail2.eps}}
    \\
    \vspace{-3mm}
    \subfloat[\label{subfig:c}]{
        \includegraphics[width=0.5\linewidth]{Figures/detail4.eps} }
    \hspace{-5mm}
    \subfloat[\label{subfig:d}]{
        \includegraphics[width=0.5\linewidth]{Figures/detail3.eps}}
    \vspace{-0.3cm}
    \caption{Top-1 accuracy under different hyperparameters: (a) batch size (b) the number of in-batch negative (c) weight of triplet loss $\lambda_t$ (d) weight of contrastive loss $\lambda_c$ .}
    \label{fig:details}
\end{figure}

==> Tables/entity.tex <==
\begin{table}[htbp]
    \renewcommand\arraystretch{1}
    \footnotesize
    \centering
    \caption{Entity representation: previous and enhanced (Now).}
    \vspace{-0.3cm}
    \label{tab:entity}
    \begin{tabular}{p{0.35cm}p{3.5cm}p{3.5cm}}
        \hline
        % \begin{minipage}[c]{0.45\linewidth} Image\end{minipage}
        %  & \makebox[5cm][c]{\begin{minipage}[c]{0.37\linewidth}\centering{\includegraphics[width=\linewidth]{Figures/Sirleaf.jpg}}\end{minipage} }                     \\
        % Text     & Sirleaf with U.S.Secretary of State Hillary Clinton.             \\
        % Mention  & Sirleaf                                                                                       \\
        \textbf{Name}   &  Donald Trump                   &  Mike Pompeo  \\
        \hline
        \textbf{Prev} & Sex: male. Birth: 1946, Religion: Presbyterianism. Occupation: business magnate, entrepreneur, politician. Languages: English.... & Sex: male. Birth: 1963. Religion: Presbyterianism. Occupation: business executive, lawyer, politician. Languages: English... \\
        \hline
        \textbf{Now}    & Donald John Trump (born June 14, 1946) is an American politician, media personality, and businessman who served as the 45th president of the United States from 2017... & Michael Richard Pompeo is an American politician, former lawyer, and businessman who served under President Donald Trump as director of the Central Intelligence Agency... \\
        \hline
    \end{tabular}
\end{table}
